Irreversible Samplers from Jump and Continuous Markov Processes

In this paper, we propose irreversible versions of the Metropolis Hastings (MH) and Metropolis adjusted Langevin algorithm (MALA) with a main focus on the latter. For the former, we show how one can simply switch between different proposal and acceptance distributions upon rejection to obtain an irreversible jump sampler (I-Jump). The resulting algorithm has a simple implementation akin to MH, but with the demonstrated benefits of irreversibility. We then show how the previously proposed MALA method can also be extended to exploit irreversible stochastic dynamics as proposal distributions in the I-Jump sampler. Our experiments explore how irreversibility can increase the efficiency of the samplers in different situations.

==> Scalable.tex <==
\section{Scaling Up the Sampling Algorithms for Large Datasets}
\label{sec:scaling}
We wish to scale up the previously discussed sampling algorithms to cases where our target distribution is a posterior distribution in a Bayesian model, and we are faced with a huge number of observations $\mathcal{S}$.
In this case, the likelihood, or its gradient, can be computationally prohibitive to compute.
In the cases of i.i.d. data, we write our target distribution as $\pi(\theta) = p(\mathcal{S} | \theta) \ p(\theta) = \prod_{{\bf s} \in \mathcal{S}} p({\bf s} | \theta) \ p(\theta)$.
For the samplers designed from continuous dynamics (Section~\ref{sec:cont}), we can use \emph{stochastic gradients}, in place of the full data gradient as elaborated in \cite{completesample} and outlined below.
For samplers using jump processes (Section~\ref{sec:jump}), we discuss a generalization of the subsampling-within-MH ideas in \cite{Korattikara:2013austerity,Bardenet,TallData}.

\paragraph{Stochastic Gradient Samplers}
For samplers using continuous dynamics \eqref{Eq:SDE}, the computationally intensive component in the update rule of \eqref{Eq:simple-update}
is the computation of
%$\nabla H(\vz_t)$, which can be explained as follows.
%Assume that the data ${\bf s} \in \mathcal{S}$ are i.i.d.: ${\bf s} \sim p({\bf s}| \theta)$.  We write our posterior distribution as $p(\theta|\mathcal{S}) \propto \exp(-U(\theta))$, where the \emph{potential function} $U$ is given by
%%
%$
%U(\theta) = - \sum_{{\bf s}\in \mathcal{S}} \log p({\bf s}|\theta) - \log p(\theta).
%$
%Recall that we have set our total target distribution as: $\pi(\vz) = p(\mathcal{S} | \theta) \ p(r)$.
%Hence, $H(\vz) = U(\theta) + \ln p(r)$.
%%
%Calculating the gradient of $H(\vz)$ involves evaluating the gradient of $U(\theta)$.
%That is:
$\nabla H(\theta) = - \nabla\log \pi(\theta) = - \sum_{{\bf s}\in \mathcal{S}} \nabla\log p({\bf s}|\theta) - \nabla\log p(\theta)$.
%When the amount of data is large, $U(\theta)$ can be too computationally intensive to calculate as it relies on a sum over all data points.
One idea for avoiding this per iteration cost is to use {\em stochastic gradients} instead \cite{SGD}.
Here, a noisy gradient based on a data subsample or {\em minibatch}, is used as an unbiased estimator of the full data gradient.
More formally, we examine \emph{independently sampled} minibatches $\widetilde{\mathcal{S}} \subset \mathcal{S}$.
The corresponding log-posterior for these data is
%
\begin{align}
\widetilde{H}(\theta) = -\dfrac{|\mathcal{S}|}{|\widetilde{\mathcal{S}}|} \sum_{{{\bf s}}\in \widetilde{\mathcal{S}}} \log p({{\bf s}}|\theta) - \log p(\theta); \quad \widetilde{\mathcal{S}} \subset \mathcal{S}.
\label{eqn:tildeU}
\end{align}
The specific form of \eqref{eqn:tildeU} implies that $\widetilde{H}(\theta)$ is an unbiased estimator of $H(\theta)$, thus $\nabla \widetilde{H}(\theta)$ is an unbiased estimator of $\nabla {H}(\theta)$.
%As such, a gradient computed based on $\widetilde{U}(\theta)$---called a \emph{stochastic gradient}~\cite{SGD}---is a noisy, but unbiased estimator of the full-data gradient.
The key question in many of the existing stochastic gradient MCMC algorithms is whether the noise injected by the stochastic gradient $\nabla \widetilde{H}(\theta)$ adversely affects the stationary distribution of the modified dynamics.
%(using $\nabla\widetilde{U}(\theta)$ in place of $\nabla U(\theta)$).
One way to analyze the impact of the stochastic gradient is to assume the central limit theorem holds:
%\begin{equation}
%\nabla \psU(\theta) = \nabla U(\theta ) +\mathcal{N}(0, \mV(\theta)), \label{eqn:noisygrad}
%\end{equation}
$\nabla \widetilde{H}(\theta) = \nabla H(\theta ) +\mathcal{N}(0, \mV(\theta))$.
%resulting in a noisy Hamiltonian gradient $\nabla \widetilde{H}(\vz) = \nabla H(\vz)+[\mathcal{N}(0,\mV(\theta)), \vzero]^T$.
Simply plugging in $\nabla \widetilde{H}(\theta)$ in place of $\nabla H(\theta)$ in \eqref{Eq:simple-update} results in dynamics with an additional noise term $({\mD}(\theta_t) + {\mQ}(\theta_t)\big)[\mathcal{N}(0,\mV(\theta_t))]^T$.
%
In our earlier work \cite{completesample}, we studied the influence of this noise and showed that one may counteract it by assuming an estimate $\hat{\mB}_t$ of the noise variance and following:
%To counteract this, assume we have an estimate $\hat{\mB}_t$ of the variance of this additional noise satisfying $2\mD(\vz_t) - \eps_t \hat{\mB}_t \succeq 0$ (i.e., positive semidefinite).
%With small $\epsilon$, this is always true since the stochastic gradient noise %$\eps \mV(\theta)$
%scales down faster than the added noise.
%Then, we can attempt to account for the stochastic gradient noise by simulating
\begin{equation}
%\begin{tiny}
    \vz_{t+1} \leftarrow \vz_{t} -  \eps_t \left[\big({\mD}(\vz_t) + {\mQ}(\vz_t)\big) \nabla \widetilde{H}(\vz_t)
+ \Gamma(\vz_t)\right] + \mathcal{N}(0, \eps_t (2\mD(\vz_t) - \eps_t \hat{\mB}_t)).  \label{Eq:true-update}
%\end{tiny}
\end{equation}
In the limit of $\eps_t$ going to zero, the stationary distribution is preserved.
For finite $\eps_t$, a bias exists.
The same bias-speed tradeoff was used in past stochastic gradient sampling methods \cite{SGLD,SGHMC,SGNHT,Shang}.
In \cite{completesample}, we also devise methods for defining new samplers using existing $\mD$ and $\mQ$ matrices as building blocks.
As a specific example, we consider a Riemann version of SGHMC method \cite{SGHMC}, and demonstrated the gains over existing benchmarks on a large streaming Wikipedia analysis.
%Comparing to the original update rule in Eq.~\eqref{Eq:SDE}, the full data gradient is replaced by the stochastic gradient, and the variance of the injected noise is subtracted by $\eps_t \hat{\mB}_t$.
%This provides our \textbf{stochastic gradient}---or \emph{\textbf{minibatch}}--- variant of the sampler.  In Eq.~\eqref{Eq:true-update}, the noise introduced by the stochastic gradient is multiplied by $\eps_t$ (and the compensation by $\eps_t^2$), implying that the discrepancy between these dynamics and those of Eq.~\eqref{Eq:simple-update} approaches zero as $\eps_t$ goes to zero. As such, in this infinitesimal step size limit, since Eq.~\eqref{Eq:simple-update} yields the correct invariant distribution, so does Eq.~\eqref{Eq:true-update}.
%This avoids the need for a costly or potentially intractable MH correction.  However, having to decrease $\eps_t$ to zero comes at the cost of increasingly small updates. We can also use a finite, small step size in practice, resulting in a biased~(but faster) sampler.
%A similar bias-speed tradeoff was used in~\cite{Korattikara:2013austerity,Bardenet,TallData} to construct MH samplers (see Section~\ref{sec:subsampler_jump}), in addition to being used in SGLD and SGHMC.
For the irreversible (and reversible) MALA algorithms, if an accurate estimate of the stochastic gradient noise is available, the stochastic gradient method can be combined with the subsampling approach described below to provide scalable variants of the MALA algorithms.


\paragraph{Subsampling of Irreversible Sampler from Jump Processes}
\label{sec:subsampler_jump}
For the irreversible jump sampler (Algorithm~\ref{alg:IrrMC}),
we can directly generalize the subsampling idea for the MH algorithms \cite{Korattikara:2013austerity}
and its adaptive and proxy method variations \cite{Bardenet,TallData}.
%
In Algorithm~\ref{alg:IrrMC}, the computational bottleneck is at the step where we decide to accept or reject the proposal from $\widetilde{f}\left(\theta(*), \theta^p(*) | \theta{(t)}, \theta^p{(t)} \right)$,
since we need to calculate $\pi(\theta(*))/\pi(\theta(t))$, requiring evaluation of the entire likelihood.

The accept-reject step is then implemented by sampling a uniform random variable $u \sim \mathcal{U}_{[0,1]}$ and accepting the proposal if and only if
%\begin{align}
%u<\dfrac{ \pi\left(\theta(*)\right) \pi\left(\theta^p(*)\right) \widetilde{g}\left(\theta{(t)}, \theta^p{(t)} | \theta(*), \theta^p(*) \right)}
%  { \pi\left(\theta{(t)}\right) \pi\left(\theta^p{(t)}\right) \widetilde{f}\left(\theta(*), \theta^p(*) | \theta{(t)}, \theta^p{(t)} \right)}.
%\end{align}
$u<\alpha\left( \theta(t), \theta^p(t), \theta(*), \theta^p(*) \right)$.
%
Following \cite{Korattikara:2013austerity,Bardenet}, we can rewrite this condition as:
%
%Recall that our target distribution in the case of i.i.d. data decomposes as: $\pi(\theta) = p(\mathcal{S} | \theta) \ p(\theta) = \prod_{{\bf s} \in \mathcal{S}} p({\bf s} | \theta) \ p(\theta)$.
%Therefore, similar to the references \cite{Korattikara:2013austerity,Bardenet}, the above Eq.~\eqref{eq:acc_cond} can be written as:
\begin{align}
\Lambda_{\mathcal{S}}(\theta(t),\theta(*)) > \Theta_{\mathcal{S}} (u, \theta(t), \theta(*), \theta^p(t), \theta^p(*)), \label{eq:acc_cond}
\end{align}
where
\begin{align}
\Lambda_{\mathcal{S}}(\theta(t),\theta(*)) &= \dfrac{1}{|\mathcal{S}|} \sum_{{\bf s} \in \mathcal{S}} \log\left[\dfrac{p({\bf s} | \theta(*))}{p({\bf s} | \theta(t))}\right], \nonumber\\
%\end{align}
%and
%\begin{align}
\Theta_{\mathcal{S}}(u, \theta(t), \theta(*), \theta^p(t), \theta^p(*)) &= \dfrac{1}{|\mathcal{S}|} \log\left[ u
\dfrac{ \pi\left(\theta^p{(t)}\right) \widetilde{f}\left(\theta(*), \theta^p(*) | \theta{(t)}, \theta^p{(t)} \right) }
{ \pi\left(\theta^p(*)\right) \widetilde{g}\left(\theta{(t)}, \theta^p{(t)} | \theta(*), \theta^p(*)\right) }
\right].
\nonumber
\end{align}
For the computationally intractable $\Lambda_{\mathcal{S}}(\theta(t),\theta(*))$, we can use a subset of data to approximate it via:
\begin{align}
\Lambda^*_{\widetilde{\mathcal{S}}}(\theta(t),\theta(*)) = \dfrac{1}{|\widetilde{\mathcal{S}}|} \sum_{{\bf s} \in \widetilde{\mathcal{S}}}
\log\left[\dfrac{p({\bf s} | \theta(*))}{p({\bf s} | \theta(t))}\right]
\approx \Lambda_{\mathcal{S}}(\theta(t),\theta(*)); \quad \widetilde{\mathcal{S}} \subset \mathcal{S}.
\nonumber
\end{align}
Importantly,
$| \Lambda_{\mathcal{S}}(\theta(t),\theta(*)) - \Lambda^*_{\widetilde{\mathcal{S}}}(\theta(t),\theta(*)) |$
can be bounded probabilistically \cite{Bardenet}.
Hence, a speed-bias tradeoff can be quantified through the probabilistic bounds when we use $\Lambda^*_{\widetilde{\mathcal{S}}}(\theta(t),\theta(*))$ instead of $\Lambda_{\mathcal{S}}(\theta(t),\theta(*))$.
%to compare with $\Theta_{\mathcal{S}}(u, \theta(t), \theta(*), \theta^p(t), \theta^p(*))$.
In some cases, more data can be used to tighten or approximate the bound on
$| \Lambda_{\mathcal{S}}(\theta(t),\theta(*)) - \Lambda^*_{\widetilde{\mathcal{S}}}(\theta(t),\theta(*)) |$, so that inequality~\eqref{eq:acc_cond} can always be verified.
Then the above procedure still yields an exact sampler.
In many cases, however, so much data has to be used that the computation gains of subsampling are negligible.
As such, we typically view this scheme as one with quantifiable bias.
See \cite{TallData} for further discussions and developments.

%Our irreversible sampler of Algorithm \ref{alg:IrrMC} is implemented in the same manner as the MH algorithm.
%a lot of improvements on the original Metropolis-Hastings algorithm can be directly applied to the irreversible sampler and make it even more efficient and scalable
%in specific problems (e.g., combining the irreversible jump sampler with RAM algorithm can possibly lead to more exploration power for multimodal distributions).
Overall, due to the similarities between our irreversible jump sampler and the MH algorithm, many methods developed specifically for MH can be applied in our context, which is quite appealing.
For example, as discussed above, we have directly applied the subsampling approach designed for scaling MH to our approach.
We can also combine our irreversible jump sampler with the RAM algorithm to further improve exploration in the case of multimodal targets.


%\subsection{Experiments}
%In Section~\ref{sec:sim}, we show that gSGRHMC can excel at rapidly exploring distributions with complex landscapes.  We then apply SGRHMC to sampling in a latent Dirichlet allocation (LDA) model on a large Wikipedia dataset in Section~\ref{sec:LDA}. Appendix~\ref{supp:Parameters} contains details on the specific samplers considered and the parameter settings used in these experiments.
%
%
%\subsubsection{Synthetic Experiments}
%\label{sec:sim}
%\begin{figure}[t!]
%\centering
%\includegraphics[height=0.17\textheight]{figure/ErrorAll_TVD.eps}
%\includegraphics[height=0.2\textheight]{figure/OnePeaks2D2_runtime.eps}
%\hspace*{-0.5in}
%\llap{\raisebox{3cm}{%  move next graphics to top right corner
%%\llap{\raisebox{2.6cm}{%  move next graphics to top right corner
%\includegraphics[height=0.032\textheight]{figure/sgldsamples1.eps}
%\hspace*{0.05in}
%%\begin{minipage}[t][0.2\textheight][s]{0.12\textwidth}
%\begin{minipage}[t][0.2\textheight][s]{0.05\textwidth}
%  \includegraphics[height=0.0325\textheight]{figure/sghmcsamples1.eps}
%  \vspace*{-20in}
%  \includegraphics[height=0.056\textheight]{figure/gsgrhmcsamples2.eps}
%\end{minipage}
%}}
%\caption{ \emph{Left: } For two simulated 1D distributions defined by $U(\theta) = \theta^2/2$ (\emph{one peak}) and $U(\theta) = \theta^4-2\theta^2$ (\emph{two peaks}), we compare the KL divergence of methods: \textcolor[rgb]{0.0, 1.0, 1.0}{\texttt{SGLD}}, \textcolor[rgb]{0.0, 1.0, 0.0}{\texttt{SGHMC}}, the \textcolor[rgb]{0.0, 0.0, 1.0}{\texttt{na\"{i}ve SGRHMC}} of Eq.~\eqref{eq:SGRHMCnaive}, and the \textcolor[rgb]{1.0, 0.0, 0.0}{\texttt{gSGRHMC}} of Eq.~\eqref{ExSGRHMC} relative to the true distribution in each scenario (left and right bars labeled by $1$ and $2$). \emph{Right: } For a correlated 2D distribution with $U(\theta_1,\theta_2) = \theta_1^4/10 + (4\cdot(\theta_2+1.2) - \theta_1^2)^2/2$, we see that our \textcolor[rgb]{1.0, 0.0, 0.0}{\texttt{gSGRHMC}} most rapidly explores the space relative to \textcolor[rgb]{0.0, 1.0, 0.0}{\texttt{SGHMC}} and \textcolor[rgb]{0.0, 1.0, 1.0}{\texttt{SGLD}}.  Contour plots of the distribution along with paths of the first 10 sampled points are shown for each method.}
%\label{fig:sim}
%\end{figure}
%In this section we aim to empirically (i) validate the correctness of our recipe and (ii) assess the effectiveness of gSGRHMC.
%In Fig.~\ref{fig:sim}(left), we consider two univariate distributions (shown in the Supplement) and compare SGLD, SGHMC, the na\"{i}ve state-adaptive SGHMC of Eq.~\eqref{eq:SGRHMCnaive}, and our proposed gSGRHMC of Eq.~\eqref{ExSGRHMC}. See the Supplement for the form of $\mG(\theta)$. As expected, the na\"{i}ve implementation does not converge to the target distribution. In contrast, the gSGRHMC algorithm obtained via our recipe indeed has the correct invariant distribution and efficiently explores the distributions.
%In the second experiment, we sample a bivariate distribution with strong correlation. The results are shown in Fig.~\ref{fig:sim}(right). The comparison between SGLD, SGHMC, and our gSGRHMC method shows that both a state-dependent preconditioner and Hamiltonian dynamics help to make the sampler more efficient than either element on its own. %gSGRHMC, which combines both element explores the space more effectively.
%
%%\begin{figure}%
%%\vspace{-10pt}
%%%\hspace{-15pt}
%%%\centering
%%%\hspace{-2pt}
%%\parbox{0.4\textwidth}{
%%\begin{footnotesize}
%%\tabcolsep=0.11cm
%%\begin{tabular}{ l | c  c } %\hline
%%\ & {\bf Original LDA} & {\bf Expanded Mean}\\
%%Parameter $\theta$ & $\beta_{kw} = \theta_{kw}$ & $\beta_{kw}=\frac{\theta_{kw}}{\sum_w \theta_{kw}}$\\
%%Prior $p(\theta)$ & $p(\theta_k) = {\rm Dir}(\alpha)$ & $p(\theta_{kw}) = \Gamma(\alpha,1)$ %\\
%%\end{tabular}\\[24pt]
%%\begin{tabular}{ l | c } %\hline
%%{\bf Method} \quad \hspace{1.5pt} & \quad {\bf Average Runtime per 100 Docs}\\
%%\textcolor[rgb]{0.0, 1.0, 1.0}{\texttt{SGLD}} & 0.778s\\
%%\textcolor[rgb]{0.0, 1.0, 0.0}{\texttt{SGHMC}} & 0.815s\\
%%\textcolor[rgb]{0.0, 0.0, 1.0}{\texttt{SGRLD}} & 0.730s\\
%%\textcolor[rgb]{1.0, 0.0, 0.0}{\texttt{SGRHMC}} & 0.806s\\
%%\end{tabular}
%%\end{footnotesize}
%%}
%%%\qquad\quad
%%%\hspace{\fill}
%%\hspace{0.2pt}
%%\begin{minipage}[c]{0.5\textwidth}%
%%%\hspace{\fill}
%%    \includegraphics[width=3in]{figure/NewPerplexity2.eps}
%%\end{minipage}
%%\hspace{-8pt}
%%\caption{\small \emph{Upper Left:} Expanded mean parameterization of the LDA model.
%%\emph{Lower Left:} Average runtime per 100 Wikipedia entries for all methods.
%%\emph{Right:} Perplexity versus number of Wikipedia entries processed.}
%%\label{fig:lda}
%%\end{figure}
%
%\begin{figure}%
%\centering
%%\parbox{0.4\textwidth}{
%%\tabcolsep=0.11cm
%\begin{tabular}{ l | c  c } %\hline
%\ & {\bf Original LDA} & {\bf Expanded Mean}\\
%Parameter $\theta$ & $\beta_{kw} = \theta_{kw}$ & $\beta_{kw}=\frac{\theta_{kw}}{\sum_w \theta_{kw}}$\\
%Prior $p(\theta)$ & $p(\theta_k) = {\rm Dir}(\alpha)$ & $p(\theta_{kw}) = \Gamma(\alpha,1)$ %\\
%\end{tabular}\\[24pt]
%\begin{tabular}{ l | c } %\hline
%{\bf Method} \quad \hspace{1.5pt} & \quad {\bf Average Runtime per 100 Docs}\\
%\textcolor[rgb]{0.0, 1.0, 1.0}{\texttt{SGLD}} & 0.778s\\
%\textcolor[rgb]{0.0, 1.0, 0.0}{\texttt{SGHMC}} & 0.815s\\
%\textcolor[rgb]{0.0, 0.0, 1.0}{\texttt{SGRLD}} & 0.730s\\
%\textcolor[rgb]{1.0, 0.0, 0.0}{\texttt{SGRHMC}} & 0.806s\\
%\end{tabular}
%%}
%\\
%\includegraphics[width=3.5in]{figure/NewPerplexity2.eps}
%\caption{\emph{Top:} Expanded mean parameterization of the LDA model.
%\emph{Middle:} Average runtime per 100 Wikipedia entries for all methods.
%\emph{Bottom:} Perplexity versus number of Wikipedia entries processed.}
%\label{fig:lda}
%\end{figure}
%
%\subsubsection{Online Latent Dirichlet Allocation}
%\label{sec:LDA}
%We also applied SGRHMC (with ${\mG}(\theta) = {\rm diag}(\theta)^{-1}$, the Fisher information metric) to an \emph{online} latent Dirichlet allocation (LDA)~\cite{Blei:2003:LDA} analysis of topics present in Wikipedia entries. In LDA, each topic is associated with a distribution over words, with $\beta_{kw}$ the probability of word $w$ under topic $k$.  Each document is comprised of a mixture of topics, with $\pi^{(d)}_k$ the probability of topic $k$ in document $d$. Documents are generated by first selecting a topic $z_j^{(d)} \sim \pi^{(d)}$ for the $j$th word and then drawing the specific word from the topic as $x_j^{(d)} \sim \beta_{z_j^{(d)}}$.  Typically, $\pi^{(d)}$ and $\beta_k$ are given Dirichlet priors.
%
%The goal of our analysis here is inference of the corpus-wide topic distributions $\beta_k$. Since the Wikipedia dataset is large and continually growing with new articles, it is not practical to carry out this task over the whole dataset. Instead, we scrape the corpus from Wikipedia in a streaming manner and sample parameters based on minibatches of data. Following the approach in~\cite{SGRLD}, we first analytically marginalize the document distributions $\pi^{(d)}$ and, to resolve the boundary issue posed by the Dirichlet posterior of $\beta_k$ defined on the probability simplex, use an expanded mean parameterization shown in Figure~\ref{fig:lda}(upper left).  Under this parameterization, we then compute $\nabla \log p(\theta | \vx)$ and, in our implementation, use boundary reflection to ensure the positivity of parameters $\theta_{kw}$. The necessary expectation over word-specific topic indicators $z_j^{(d)}$ is approximated using Gibbs sampling separately on each document, as in~\cite{SGRLD}.  The Supplement contains further details.
%
%For all the methods, we report results of three random runs.
%When sampling distributions with mass concentrated over small regions, as in this application, it is important to incorporate geometric information via a Riemannian sampler~\cite{SGRLD}.  The results in Fig.~\ref{fig:lda}(right) indeed demonstrate the importance of Riemannian variants of the stochastic gradient samplers.  However, there also appears to be some benefits gained from the incorporation of the HMC term for both the Riemmannian and non-Reimannian samplers.
%The average runtime for the different methods are similar (see Fig.~\ref{fig:lda}(lower left)) since the main computational bottleneck is the gradient evaluation.
%Overall, this application serves as an important example of where our newly proposed sampler can have impact.

